The Three-Dimensional Jump Conditions for the Stokes Equations with Discontinuous Viscosity, Singular Forces, and an Incompressible Interface

The three-dimensional jump conditions for the pressure and velocity fields, up to the second normal derivative,across an incompressible/inextensible interface in the Stokes regime are derived herein. The fluid viscosity is only piecewise continuous in the domain while the embedded interface exerts singular forces on the surround fluids. This gives rise to discontinuous solutions in the pressure and velocity field. These jump conditions are required to develop accurate numerical methods, such as the Immersed Interface Method, for the solutions of the Stokes equations in such situations.

==> 05_NumericalMethod.tex <==
\section{\label{sec:NumericalMethod} Numerical Method}

In this section, the numerical implementation and the algorithm is explained in detail. The
method here follows that given in Ref. \cite{Tan20089955}. Here the 
singular force given in Eq. (\ref{eq:singular_forces}) will be considered. On a given computational domain
the augmented equations, (\ref{eq:augmented_momentum}) and (\ref{eq:augmented_pressure}), can be written in linear 
operator form. As all of the jump conditions are linear, then so will the IIM corrections near the interface.
Letting the vectors $\vec{q}$, $\vec{\gamma}$, and 
$\vec{f}_0$ contain the interface velocity, surface tension, and singular force, for the entire domain it is possible
to write the corrections as $\vec{C}_p=\vec{A}_0\vec{q}+\vec{B}_0\vec{\gamma}+\vec{C}_0\vec{f}_0$ and
$\vec{C}_u=\vec{A}_1\vec{q}+\vec{B}_1\vec{\gamma}+\vec{C}_1\vec{f}_0$. Thus 
\begin{align}
	\label{eq:lop1} \vec{L p}&=\vec{Dg}+\vec{A}_0\vec{q}+\vec{B}_0\vec{\gamma}+\vec{C}_0\vec{f}_0, \\
	\label{eq:lop2} \vec{L \wt{u}}&=\vec{Gp}-\vec{g}+\vec{A}_1\vec{q}+\vec{B}_1\vec{\gamma}+\vec{C}_1\vec{f}_0,
\end{align}
where $\vec{L}$, $\vec{D}$, and $\vec{G}$ are the Laplacian, divergence, and gradient operators, respectively. 

Solving Eq. (\ref{eq:lop1}) for the pressure it is possible to write the velocity field as
\begin{align}
	\vec{\wt{u}}=&
	\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{D}-\vec{I}\right)\vec{g} \nonumber\\
	&\qquad+\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{C}_0+\vec{C}_1\right)\vec{f}_0 \nonumber \\
	&\qquad+\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{A}_0+\vec{A}_1\right)\vec{q} \nonumber \\
	&\qquad+\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{B}_0+\vec{B}_1\right)\vec{\gamma}
\end{align}

Introducing the operator $\vec{M}$, which interpolates onto the interface such that $\vec{M\wt{u}}=\vec{q}$, it is possible to write
\begin{align}
	\vec{q}=&
	\vec{M}\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{D}-\vec{I}\right)\vec{g} \nonumber \\
	&\qquad+\vec{M}\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{C}_0+\vec{C}_1\right)\vec{f}_0+\vec{C}_2\vec{f}_0 \nonumber \\
	&\qquad+\vec{M}\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{A}_0+\vec{A}_1\right)\vec{q}+\vec{A}_2\vec{q} \nonumber \\
	&\qquad+\vec{M}\vec{L}^{-1}\left(\vec{G}\vec{L}^{-1}\vec{B}_0+\vec{B}_1\right)\vec{\gamma}+\vec{B}_2\vec{\gamma},
\end{align}
where $\vec{A}_2\vec{q}+\vec{B}_2\vec{\gamma}+\vec{C}_2\vec{f}_0$ are the corrections needed for the interpolation operator.
	
It is possible to write this system in simplified form as
\begin{equation}
	\label{eq:sys1}
	\vec{q}=\vec{q}_0+\vec{Aq}+\vec{B\gamma}.
\end{equation}
In this expression $\vec{q}_0$ represents the velocity on the interface due to only the body force $\vec{g}$ and the singular 
force $\vec{f}_0$. Similarly the matrix-vector product $\vec{Aq}$ and $\vec{B\gamma}$ are the velocities on the interface
due to only the quantities $\vec{q}$ and $\gamma$. Eq. \ref{eq:sys1} simply indicates that the total velocity on
the interface has three contributions: known forces, contributions from the velocity itself, and the interfacial tension.

In Eq. (\ref{eq:sys1}) there are two unknowns, the interfacial velocity $\vec{q}$ and tension $\vec{\gamma}$. The 
tension acts as a Lagrange multiplier and will be used to enforce surface incompressibility. To obtain a second 
equation let the linear operator $\vec{D}_s$ represent the surface divergence of a vector field on the interface. 
Applying the surface divergence operator and noting that $\vec{D}_s\vec{q}=0$ a second equation can be obtained:
\begin{equation}
	\label{eq:sys2}
	0=\vec{D}_s\vec{q}_0+\vec{D}_s\vec{Aq}+\vec{D}_s\vec{B\gamma}.
\end{equation}

Equations (\ref{eq:sys1}) and (\ref{eq:sys2}) can be written in block-matrix form as
\begin{equation}
	\label{eq:blocksys}
	\begin{pmatrix}
		\vec{A}-\vec{I} & \vec{B} \\
		\vec{D}_s\vec{A} & \vec{D}_s\vec{B}
	\end{pmatrix}
	\begin{pmatrix}
		\vec{q} \\
		\vec{\gamma}
	\end{pmatrix} = 
	\begin{pmatrix}
		-\vec{q}_0 \\
		-\vec{D}_s\vec{q}_0
	\end{pmatrix}.
\end{equation}
As it is not feasible to explicitly form the matrices $\vec{A}$ or $\vec{B}$ a matrix-free iterative solver, such as GMRES, is needed 
to solve the given linear system.


\subsection*{Algorithm}
The algorithm and boundary conditions needed to solve Eq. (\ref{eq:blocksys}) is outlined here. This algorithm will be used 
below to solve sample problems and verify the accuracy of the method.

\begin{enumerate}[I.]
	\item{
		Compute the quantities $\vec{q}_0$ and $\vec{D}_s\vec{q}_0$. For this step all jump conditions are 
		calculated using only $\vec{g}$ and $\vec{f}_0$ (\textit{e.g.} assume that $\vec{q}=0$ and $\vec{\gamma}=0$).
		\begin{enumerate}[1.]
			\item{Solve Eq. (\ref{eq:augmented_pressure}) to obtain the pressure field. 
				Use Neumann boundary conditions of $\partial p/\partial n_b=\vec{n}_b\cdot\nabla^2\vec{u}_b+\vec{g}\cdot\vec{n}_b$,
				where $\vec{n}_b$ is the outward facing normal to the computational domain and $\vec{u}_b$ is the known velocity field on domain boundary.}
			\item{Solve Eq. (\ref{eq:augmented_momentum}) to obtain the velocity field. Use Dirilichet boundary conditions of $\vec{u}=\vec{u}_b$ on the domain boundary.}
			\item{Interpolate the velocity field onto the interface to obtain $\vec{q}_0$. For interpolation use a tri-cubic interpolant.}
			\item{Calculate the surface divergence of the interface velocity, $\vec{D}_s\vec{q}_0$.}
		\end{enumerate}	
	}
	\item{\label{step} Solve Eq. (\ref{eq:blocksys}) using GMRES. During each GMRES iteration a matrix-vector product operation is required.
		As the quantities $\vec{q}$ and $\vec{\gamma}$ are supplied during the iterations the following steps are performed.
		In this case all jump conditions are calculated using only $\vec{q}$ and $\vec{\gamma}$ (\textit{e.g.} assume that $\vec{g}=0$ and $\vec{f}_0=0$).
		\begin{enumerate}[1.]
			\item{The quantities $\vec{q}$ and $\vec{\gamma}$ are supplied by the GMRES solver.}
			\item{Solve Eq. (\ref{eq:augmented_pressure}) to obtain the pressure field. 
				Based on the superposition principle it is possible to use Neumann boundary conditions of $\partial p/\partial n_b=0$.}
			\item{Solve Eq. (\ref{eq:augmented_momentum}) to obtain the velocity field. Use Dirilichet boundary conditions of $\vec{u}=0$ on the domain boundary.}
			\item{Interpolate the velocity field onto the interface to obtain $\vec{A}\vec{q}+\vec{B}\vec{\gamma}$. For interpolation use a tri-cubic interpolant.}
			\item{Calculate the surface divergence of the interface velocity, $\vec{D}_s\left(\vec{A}\vec{q}+\vec{B}\vec{\gamma}\right)$. This is the second 
			component of the block matrix-vector product.}
			\item{Subtract $\vec{q}$ from $\vec{A}\vec{q}+\vec{B}\vec{\gamma}$ to obtain the first component of the block matrix-vector product.}
		\end{enumerate}
	}
\end{enumerate}
Note that in Step \ref{step} of the algorithm the quantity $\vec{Aq}+\vec{B\gamma}$ is calculated simultaneously to reduce the overall computational cost.

